From a Natural to a Formal Language with DSL Assistant

The development of domain-specific languages (DSLs) is a laborious and iterative process that seems to naturally lean to the use of generative artificial intelligence. We design and prototype DSL Assistant, a tool that integrates generative language models to support the development of DSLs. DSL Assistant uses OpenAI's assistant API with GPT-4o to generate DSL grammars and example instances. To reflect real-world use, DSL Assistant supports several different interaction modes for evolving a DSL design, and includes automatic error repair. Our experiments show that DSL Assistant helps users to create and modify DSLs. However, the quality of the generated DSLs depends on the specific domain and the followed interaction patterns.

==> fig/part1-2-agg.tex <==
\begin {table} [t]
\begin {tabular} {
  l
  c
  c
  c
  c
  c
  c
  c
  c
  c
}

   &
   &
   & \multicolumn{2}{c}{\textbf{\footnotesize Correct.}}
   & \multicolumn{5}{c}{\textbf{\footnotesize Line Diff.\ of Grammars}}
   \\

   \cline{4-5} \cline{6-10}

     \textbf {Origin}
   & \textbf {\#}
   & \textbf {\%}
   & \textbf {\#}
   & \textbf {\%}
   & \textbf {M}
   & \textbf {SD}
   & \textbf {min}
   & \textbf {max}
   & \textbf {median}
   \\

  AI
  & 44
  & 57
  & 4
  & 9
  & 3.7
  & -2
  & 58
  & 11.9
  & 0
  \\

  Human
  & 17
  & 53
  & 8
  & "\textbf{47}"
  & 5.8
  & -7
  & 46
  & 13.2
  & 0
  \\

  Total
  & 61
  & \textbf{56}
  & \textbf{12}
  & 20
  & 4.3
  & -7
  & 58
  & 12.3
  & 0
  \\

\end {tabular}

\caption {Results for \cref{sec:met-c}. Reproduced DSL version with grammar changes from part 2 including correction and differences (measured in number of lines) and grouped by origin}%
\label {tab:auto-02-part1-2-agg}

\end {table}

